Automating Software Development for Mobile Computing Platforms (Doctoral Symposium)

Mobile devices such as smartphones and tablets have become ubiquitous in today's modern computing landscape. The applications that run on these mobile devices (often referred to as "apps") have become a primary means of computing for millions of users and, as such, have garnered immense developer interest. These apps allow for unique, personal software experiences through touch-based UIs and a complex assortment of sensors. However designing and implementing high quality mobile apps can be a difficult process. This is primarily due to challenges unique to mobile development including change-prone APIs and platform fragmentation, just to name a few. This paper presents the motivation and an overview of a dissertation which presents new approaches for automating and improving mobile app design and development practices. Additionally, this paper discusses potential avenues for future research based upon the work conducted, as well as general lessons learned during the author's tenure as a doctoral student in the general areas of software engineering, maintenance, and evolution.

==> macro.tex <==
\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\useunder{\uline}{\ul}{}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}

\newcommand{\CrashScopesp}{{\sc CrashScope~}}
\newcommand{\CrashScopes}{{\sc \small CrashScope's~}}
\newcommand{\CrashDroid}{{\sc CrashDroid~}}
\newcommand{\CrashScopebf}{{ \textbf{\sc CrashScope~}}}

\newcommand{\ReDraw}{{\sc \small ReDraw}\xspace}
\newcommand{\ReDraws}{{\sc \small ReDraw's}\xspace}
\newcommand{\Remaui}{{\sc \small Remaui}\xspace}
\newcommand{\Remauis}{{\sc \small Remaui's}\xspace}
\newcommand{\CrashScope}{{\sc \small CrashScope}\xspace}
\newcommand{\MonkeyLab}{{\sc \small MonkeyLab}\xspace}
\newcommand{\pixcode}{{\small pix2code}\xspace}

\newcommand{\GVTsp}{{\sc \small Gvt~}}
\newcommand{\GVT}{{\sc \small Gvt}}
\newcommand{\GVTs}{{\sc \small Gvt's~}}
\newcommand{\GVTbf}{{ \textbf{\sc Gvt~}}}
\newcommand{\dv}{{\textit{DV}}\xspace}
\newcommand{\dvs}{{\textit{DVs}}\xspace}
\newcommand{\gc}{{\textit{GC}}\xspace}
\newcommand{\gcs}{{\textit{GCs}}\xspace}
\newcommand{\mgc}{{\textit{M-GC}}\xspace}
\newcommand{\mgcs}{{\textit{M-GCs}}\xspace}
\newcommand{\igc}{{\textit{I-GC}}\xspace}
\newcommand{\igcs}{{\textit{I-GCs}}\xspace}


\newcommand{\ReDrawAbs}{{R}{\ssmall E}{D}{\ssmall RAW}\xspace}




\newsavebox\CBox
\newlength\CLength
\def\circled#1{\sbox\CBox{#1}%
  \ifdim\wd\CBox>\ht\CBox \CLength=\wd\CBox\else\CLength=\ht\CBox\fi
    \makebox[1.2\CLength]{\makebox(0,0.9\CLength){\put(0,0){\circle{1.3\CLength}}}%
    \makebox(0,1.0\CLength){\put(-.5\wd\CBox,0){#1}}}}

\def\circledlong#1{\sbox\CBox{#1}%
  \ifdim\wd\CBox>\ht\CBox \CLength=\wd\CBox\else\CLength=\ht\CBox\fi
    \makebox[1.2\CLength]{\makebox(0,0.6\CLength){\put(0,0){\circle{1.3\CLength}}}%
    \makebox(0,0.6\CLength){\put(-.5\wd\CBox,0){#1}}}}

\lstset{
	basicstyle=\footnotesize\ttfamily,
	breaklines=true,
    frame=tb, % draw a frame at the top and bottom of the code block
    tabsize=4, % tab space width
    showstringspaces=false, % don't mark spaces in strings
    numbers=left, % display line numbers on the left
    commentstyle=\color{Red}, % comment color
    keywordstyle=\color{blue}, % keyword color
    stringstyle=\color{OliveGreen}, % string color
	xleftmargin=.25in %align numbers to left side
}

\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand\KEVIN[1]{{\color{blue} \nb{KEVIN}{#1}}}
\newcommand\MICHAEL[1]{{\color{blue} \nb{MICHAEL}{#1}}}
\newcommand\CARLOS[1]{{\color{blue} \nb{CARLOS}{#1}}}
\newcommand\RICHIE[1]{{\color{blue} \nb{RICHIE}{#1}}}
\newcommand\DENYS[1]{{\color{blue} \nb{DENYS}{#1}}}

\newcommand{\ie}{\textit{i.e.},\xspace}
\newcommand{\eg}{\textit{e.g.},\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}

\newcommand\NEW[1]{\nb{NEW}{#1}}

